Interference and Coverage Analysis of mmWave Inter-Vehicle Broadcast with Directional Antennas

Thanks to the availability of large bandwidth and high-gain directional antennas at the millimeter-wave (mmWave) bands, mmWave communications have been considered as one of the primary solutions to meet the high data rates needs in vehicular networks. Unicast in mmWave vehicle-to-vehicle (V2V) communications has been well-studied, but much less attention has been paid to V2V broadcast which is required by many V2V applications such as active safety. To fill the gap, this paper systematically investigates mmWave V2V broadcast by considering the unique properties of mmWave signal propagation in V2V environments as well as the impacts of directional antennas and interference. Based on widely-accepted, high-fidelity system models, we mathematically analyze the receiver-side signal-to-interference-plus-noise-ratio (SINR) and broadcast coverage, and we study the impacts of blockage, inter-vehicle distance, vehicle density and beam pattern. Through comprehensive numerical analysis, we find out that, instead of a single unique optimal beamwidth, there exists an optimal range of beamwidth, in which the beamwidths have similar performance and can maximize the coverage. We also find out that the selection of carrier sensing range plays an important role as it highly influences the performance of the whole vehicular networks. Our analysis provides unique insight into mmWave V2V broadcast, and it sheds light on designing effective V2V broadcast protocols.

==> todos.tex <==

ICC todos 
    Spell check
    

TR example: https://www.ece.iastate.edu/~hongwei/group/TR/ARA_Vision-TR.pdf


To do:
Impact of signal power (in TR)?


***
- Address comment in Section IV-B

- Need to find optimal value => impact of using optimal value  

- Why meaningful when only considering lane-directions of main lobe center direction? 

%- Instead of 3-lane road, consider general multi-lane road section. 

%- Figure 7: redraw the figure by only considering the receivers whose SINR is above the required threshold 23dB. 

%-* Run simulation to corroborate analytical results, those on broadcast coverage. 

*** before 4/29/21 *** 
- Interferance calculation: considering additive interference from far away regions and stochastic geometry? 

- Another way of strengthening the study is going back to the questions we were asking very early on: given the specific broadcast requirement in URLCC V2X applications (e.g., broadcast to vehicles within a fixed distance, e.g., 300 meters, with reliability/receiver-side-SINR no less than a threshold), analyze the broadcast latency and throughput, as a way for providing insight into the final algorithm design. Of course, this may or may not show up in a 6-page paper, and may not be a main focus for catching Globecom deadline (if there is time extension). 

- Urban settings, in addition to highways?

%- how is the 10dB threshold value chosen? What if a different threshold value is chosen? Perhaps you can show the impact of SINR threshold too since that reflects application requirement

%find the right modulation mode, check SINRvsBER, find the right BER, get and try min mid max SINR

%- figure 5 may want to show the case of some small bandwidths (less than 60 degrees) to differentiate more ...

